Steinberg's theorem for crystallographic complex reflection groups

Popov classified crystallographic complex reflection groups by determining lattices they stabilize. These analogs of affine Weyl groups have infinite order and are generated by reflections about affine hyperplanes; most arise as the semi-direct product of a finite complex reflection group and a full rank lattice. Steinberg's fixed point theorem asserts that the regular orbits under the action of a reflection group are exactly the orbits lying off of reflecting hyperplanes. This theorem holds for finite reflection groups (real or complex) and also affine Weyl groups but fails for some crystallographic complex reflection groups. We determine when Steinberg's theorem holds for the infinite family of crystallographic complex reflection groups. We include crystallographic groups built on finite Coxeter groups.

==> layout.tex <==
% \ifdraft{\date{\today}}{\date{}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% MISC

%\linespread{1.08}

% package lineno must be activated
%\linenumbers

% avoid line breakes
%\sloppy

% add space after punctuation marks.
%\nonfrenchspacing

% itemization spacing for package enumitem
%\setitemize{itemsep=0.05em}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% PAGE HEADERS

% \pagestyle{scrheadings}
% \clearscrheadings
% \automark[section]{subsection}
% \renewcommand{\sectionmark}[1]{\markright{Section~\thesection}}

% \cfoot[--\,\pagemark\,--]{--\,\pagemark\,--}
% \lohead{\headertitle --- \rightmark}
% \rohead{\headerauthors}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION TITLES

% \titleformat{\section}[hang]
% {\Large\sffamily\bfseries}
% {\thesection\hspace{0.1em}{|}}{0.25em}{}


% \titleformat{\subsection}[wrap]
% {\normalfont\bfseries\selectfont\filright}
% {\thesubsection\hspace{.1em}|}{.25em}{}
% \titlespacing{\subsection}
% {16pc}{1.5ex plus .1ex minus .2ex}{1pc}

% % \titleformat{\subsection}[runin]
% % {\normalfont\bfseries}
% % {\thesubsection\hspace{.1em}|}{0.25em}{}[.\hspace*{.5em}]


% \titleformat{\subsubsection}[runin]
% {\normalfont\bfseries}
% {\thesubsubsection\hspace{.1em}|}{0.25em}{}[.]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% THEOREM LIKE ENVIRONMENTS

% \renewcommand{\proofSymbol}{\rule{1ex}{1ex}}

\numberwithin{equation}{section}

\newtheorem{theoremcounter}{theoremcounter}[section]

\newtheorem{assumption}[theoremcounter]{Assumption}
\newtheorem{axiom}[theoremcounter]{Axiom}
\newtheorem{claim}[theoremcounter]{Claim}
\newtheorem{conjecture}[theoremcounter]{Conjecture}
\newtheorem{corollary}[theoremcounter]{Corollary}
\newtheorem{definition}[theoremcounter]{Definition}
\newtheorem{example}[theoremcounter]{Example}
\newtheorem{exercise}[theoremcounter]{Exercise}
\newtheorem{lemma}[theoremcounter]{Lemma}
\newtheorem{notation}[theoremcounter]{Notation}
\newtheorem{proposition}[theoremcounter]{Proposition}
\newtheorem{remark}[theoremcounter]{Remark}
\newtheorem{remarks}[theoremcounter]{Remarks}
\newtheorem{theorem}[theoremcounter]{Theorem}

\newtheorem*{remarkcomputation}{Computation}

%% ANNE'S SHORTCUTS

\newtheorem{cor}[theoremcounter]{Corollary}
\newtheorem{prop}[theoremcounter]{Proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ENUMERATION

\newenvironment{enumeratearabic}{
\begin{enumerate}[label=(\arabic*), leftmargin=0pt,labelindent=2em,itemindent=!]
}{
\end{enumerate}
}

\newenvironment{enumerateroman}{
\begin{enumerate}[label=(\roman*), leftmargin=0pt,labelindent=2em,itemindent=!]
}{
\end{enumerate}
}

\newenvironment{enumeratearabic*}{
\begin{enumerate*}[label=(\arabic*)] %%, leftmargin=0pt,labelindent=2em,itemindent=!]
}{
\end{enumerate*}
}

\newenvironment{enumerateroman*}{
\begin{enumerate*}[label=(\roman*)] %%, leftmargin=0pt,labelindent=2em,itemindent=!]
}{
\end{enumerate*}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% PYTHON KEYWORDS FOR ALGORITHM2E

% \SetStartEndCondition{ }{}{}%

% \SetKwProg{Pydef}{def}{\string:}{}
% \SetKwComment{tcc}{\#\ }{}

% \SetKwFor{For}{for}{\string:}{}%
% \SetKwFor{While}{while}{:}{fintq}%
% \SetKwIF{If}{ElseIf}{Else}{if}{:}{elif}{else:}{}%

% \SetKwFunction{Range}{range}%%
% \SetKw{KwIn}{in}
% \SetKw{KwNot}{not}
% \SetKw{KwOr}{or}
% \SetKw{KwInlineIf}{if}

% \AlgoDontDisplayBlockMarkers\SetAlgoNoEnd\SetAlgoNoLine%

